A Theory of Multimodal Learning

Human perception of the empirical world involves recognizing the diverse appearances, or 'modalities', of underlying objects. Despite the longstanding consideration of this perspective in philosophy and cognitive science, the study of multimodality remains relatively under-explored within the field of machine learning. Nevertheless, current studies of multimodal machine learning are limited to empirical practices, lacking theoretical foundations beyond heuristic arguments. An intriguing finding from the practice of multimodal learning is that a model trained on multiple modalities can outperform a finely-tuned unimodal model, even on unimodal tasks. This paper provides a theoretical framework that explains this phenomenon, by studying generalization properties of multimodal learning algorithms. We demonstrate that multimodal learning allows for a superior generalization bound compared to unimodal learning, up to a factor of $O(\sqrt{n})$, where $n$ represents the sample size. Such advantage occurs when both connection and heterogeneity exist between the modalities.

==> LTL.tex <==
\section{The Benefit in Learning to Learn}
\zl{no need to re-learn the link for a new task}

==> backup.tex <==
We consider the following decomposition:
\begin{align*}
    &R_{\mathcal{X}}(\hat{g},\hat{f}_1,...,\hat{f}_T)-R^*_{\mathcal{X}}\\
    =& \left( \frac{1}{T}\sum_{t=1}^T  \mathbb{E}_{(x,y,z)\sim \mu_t} \ell(\hat{f}_t(x,\hat{g}(x)),z)-\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n \ell(\hat{f}_t(x_{ti},\hat{g}(x_{ti})),z_{ti}) \right)\\
    +& \left( \frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n \ell(\hat{f}_t(x_{ti},\hat{g}(x_{ti})),z_{ti})-\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n \ell(\tilde{f}_t(x_{ti},\tilde{g}(x_{ti})),z_{ti})\right)\\
    +& \left(\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n \ell(\tilde{f}_t(x_{ti},\tilde{g}(x_{ti})),z_{ti})-\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n \ell(f^*_t(x_{ti},g^*(x_{ti})),z_{ti}) \right)\\
    +& \left(\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n \ell(f^*_t(x_{ti},g^*(x_{ti})),z_{ti})- \frac{1}{T}\sum_{t=1}^T  \mathbb{E}_{(x,y,z)\sim \mu_t} \ell(f^*_t(x,g^*(x)),z)\right)
\end{align*}

We bound the first part by Gaussian averages, which is the main part of proof. The second part is assumed to be zero by the expressivity assumption \zl{can we get better?}. The third part is non-positive by definition. The last part we bound by Hoeffding’s inequality.

\subsection{Proof of Theorem \ref{mtl}}
Define $f_t^*=\mathbf{argmin}_{f\in \mathcal{F}}\mathbb{E}_{(x,y,z)\sim \mu_t} \ell(f^*_t(x,y),z)$. We make the following decomposition:
\begin{align}
    L(\hat{g},\hat{f}_1,...,\hat{f}_T)=& \left( \frac{1}{T}\sum_{t=1}^T  \mathbb{E}_{(x,y,z)\sim \mu_t} \ell(\hat{f}_t(x,\hat{g}(x)),z)-\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n \ell(\hat{f}_t(x_{ti},\hat{g}(x_{ti})),z_{ti}) \right)\label{p1}\\
    +& \left( \frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n \ell(\hat{f}_t(x_{ti},\hat{g}(x_{ti})),z_{ti})-\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n \ell(\hat{f}_t(x_{ti},\tilde{g}(x_{ti})),z_{ti})\right)\label{p2}\\
    +& \left( \frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n \ell(\hat{f}_t(x_{ti},\tilde{g}(x_{ti})),z_{ti})-\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n \ell(\hat{f}_t(x_{ti},y_{ti}),z_{ti}) \right)\label{p3}\\
    +& \left(\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n \ell(\hat{f}_t(x_{ti},y_{ti}),z_{ti})-\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n \ell(f^*_t(x_{ti},y_{ti}),z_{ti}) \right)\label{p4}\\
    +& \left(\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n \ell(f^*_t(x_{ti},y_{ti}),z_{ti})- \frac{1}{T}\sum_{t=1}^T  \mathbb{E}_{(x,y,z)\sim \mu_t} \ell(f^*_t(x,y),z)\right)\label{p5}
\end{align}
where $\tilde{g}=\mathbf{argmin}_{g\in \mathcal{G}}\frac{1}{nT} \sum_{t=1}^T \sum_{i=1}^n \|g(x_{ti})-y_{ti}\|$.

Each term is bounded separately. Term \ref{p2} is non-positive by the optimality of $\hat{g}$. Similarly, term \ref{p4} is also non-positive. Term \ref{p3} is bounded by $L\mathcal{R}(\mathcal{G},S)$, noticing that Lipschitzness is preserved by function composition using Assumption \ref{as1} and Definition \ref{def2}
\begin{align}
&\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n \ell(\hat{f}_t(x_{ti},\tilde{g}(x_{ti})),z_{ti})-\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n \ell(\hat{f}_t(x_{ti},y_{ti}),z_{ti})\\
\le& \frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n|\hat{f}_t(x_{ti},\tilde{g}(x_{ti}))-\hat{f}_t(x_{ti},y_{ti})|\\
\le& \frac{L}{nT}\sum_{t=1}^T\sum_{i=1}^n\|\tilde{g}(x_{ti})-y_{ti}\|\le L \mathcal{R}(\mathcal{G},S).
\end{align}

We can bound term \ref{p5} by Hoeffding’s inequality, since it involves only the sum of bounded independent random variables.
To be precise, denote $v_{ti}=\ell(f^*_t(x_{ti},y_{ti}),z_{ti})$, we can check that they are independent random variables, bounded in $[0,1]$, with expectation equal to $\mathbb{E}_{(x,y,z)\sim \mu_t} \ell(f^*_t(x,y),z)$. The Hoeffding’s inequality states that for any $t>0$,
$$
\mathbb{P}\left(|\sum_{t,i} v_{ti}-\mathbb{E}[\sum_{t,i} v_{ti}]| \ge t\right)\le 2e^{-\frac{2t^2}{nT}}.
$$
Taking $t=\sqrt{\frac{nT\log(4/\delta)}{2}}$, we have that with probability at least $1-\frac{\delta}{2}$, term \ref{p5} is bounded by $\sqrt{\frac{\log(4/\delta)}{2nT}}$.

The first term \ref{p1} we can bound with chain rules for Gaussian average, for example \cite{maurer2016chain} \cite{tripuraneni2020theory}. \zl{tbd, use chi}

\begin{theorem}[\cite{bartlett2002rademacher}]
    Let $\mathcal{F}$ be a function class on $\mathcal{X}$ taking value in $[0,1]$, and let $X=\{x_1,...,x_n\}$ be a set of iid random variables from $\mathcal{X}$ and $X'$ iid to $X$. Then with probability at least $1-\delta$ in the drawing of $X$, we have that for any $f\in \mathcal{F}$
    $$
    \frac{1}{n}\sum_{i=1}^n (\mathbb{E}_{X'}[f(x'_i)]-f(x_i))\le \frac{\sqrt{2\pi}}{n} \mathbb{E}_{X} G(\mathcal{F},X)+\sqrt{\frac{9\log(2/\delta)}{2n}}.
    $$
\end{theorem}

The main difference in the setting is that, we have access to the "representations" $y$ from the training data in multimodal learning so that we can decouple the learning of $f$ and $g$. However, in representation learning we have to learn the representation from scratch. Intuitively, learning the composition $f\circ g$ can be much harder than learning them individually.

Such difference in setting leads to different methods. In representation learning we solve the ERM over the whole class of compositions $f\circ g$, while in multimodal learning we solve two ERMs separately for $f,g$ which helps us evade the worst-case Gaussian average term. We are allowed to do so because $y$ is revealed to us.

In fact, we can solve our multimodal learning problem via representation learning, by doing a naive reduction. In particular, we can directly solve the following uni-modality ERM problem by treating $y$ as a representation of $x$
$$
\hat{g},\hat{f}_1,..,\hat{f}_T=\mathbf{argmin}_{g\in \mathcal{G}, f_1,...,f_T\in \mathcal{F}} \frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n \ell(f_t(x_{ti},g(x_{ti})),z_{ti}).
$$

By classical results in representation learning, solving this ERM gives a similar bound to Theorem \ref{mtl}, except that the "empirical" Gaussian average of $\mathcal{F}$ is replaced by a worst-case quantity, as we already show in Remark \ref{rm2}. Therefore, our multimodal learning approach has an edge when $\hat{g}(x)$ nicely approximates the ground truth $y$, making $\hat{S}$ easy to learn by $\mathcal{F}$.

An illustrating example of such advantage is the following. Let $\mathcal{X}=\mathbb{R}$ and $\mathcal{Y}=\mathbb{R}^k$, we consider a distribution on $\mathcal{S}$, such that for any possible data point $(x,y,z)\in \mathcal{S}$, we have that $y=xv+y_0$ for some fixed $v,y_0\in \mathbb{R}^k$. The hypothesis classes we consider are, all $k$-degree polynomials for $\mathcal{G}$
$$
\mathcal{G}=\left\{g(x)=\sum_{i=0}^k x^i v_i|v_i\in \mathbb{R}^k\right\},
$$
and all hyperplanes for $\mathcal{F}$
$$
\mathcal{F}=\left\{f(x)=\textbf{sign}(x^{\top}v-c)|v\in \mathbb{R}^{k+1}, c\in \mathbb{R}\right\}.
$$
Take any sample $S$ with size $n\le k$. The worst case Gaussian average $\max_{g\in \mathcal{G}} G(\mathcal{F}(S(g)))$ can be as large as $\Omega(n)$, because the hypothesis class $\mathcal{F}$ is known to be able to shatter any $k$ points in $\mathbb{R}^{k+1}$ that are linearly independent, while the class $\mathcal{G}$ is expressive enough to contribute a worst-case $g$ that does map $X$ to a set of linearly independent points. However, it's possible that the learnt $\hat{g}$ is a low-dimensional polynomial. In particular, when it indeed learns the correct connection $g(x)=xv+y_0$, then the $n$ points $(x_1,\hat{g}(x_1)),...,(x_n,\hat{g}(x_n))$ are on the same line which is hard to shatter by $\mathcal{F}$, and $G(\mathcal{F}(\hat{S}))$ is just $O(\sqrt{n})$.

\begin{remark}\label{rm2}
Compared with classical bounds in representation learning, the upper bound on the order of leading terms is roughly the same: $\sqrt{\mathbf{complexity}(\mathcal{F})/n}+\sqrt{\mathbf{complexity}(\mathcal{G})/nT}$, since they usually make a realizability assumption that reduces $\mathcal{R}(\mathcal{G},S')$ to 0. However, our bound is potentially better for some instances. Due to the hardness of learning $f,g$ together, the bounds in representation learning typically include a worst case Gaussian average term, for example in \cite{tripuraneni2020theory} they have $\max_{g\in \mathcal{G}} G(\mathcal{F}(S(g)))$ instead where $S(g)=\{(x_{ti},g(x_{ti}),z)\}$ is a random set induced by $g$. As a comparison, in our bound the Gaussian average is only measured over the "instance" $\hat{S}$ which can be very small for a high-quality $\hat{g}$.
\end{remark}

\subsection{Data Separability}
The success of any machine learning application, accounts of not only a good choice of model, but also a set of suitable data. The nature of machine learning is data-dependent, and pre-processing of data is always a crucial step in practical machine learning and data science.

There have been a lot of measures on data separability, among which the linear separability is the simplest and most popular one. Numerous studies haven been made on the advantages of linear separable data, and here we focus on when multimodality can make data linearly separable through heterogeneity.

It's rather straightforward to show there are cases where $(x,y,z)$ is linearly separable while $(x,z)$ has arbitrarily complicated decision boundary even if there is a bijective mapping between $x,y$, for example using Jordan Curve Theorem in 2-d, see Figure \ref{examples}. 

\begin{figure}
    \centering
    \includegraphics[width=8cm]{multimodal 2.png}
    \caption{In the $\mathcal{Y}$ space the data is separable, while in the $\mathcal{X}$ space the decision boundary is complicated. There is a bijective mapping between $x,y$ by the definition of homeomorphism.}
    \label{examples}
\end{figure}

One may complain such complicacy originates from only the connection $g$, that one of the modality is always wasy to learn. We can construct cases where neither $\mathcal{X}$ nor $\mathcal{Y}$ itself makes data linearly separable, while together they do. The simplest case is when $\mathcal{X}=\mathcal{Y}=[0,1]$. Let $g(x): [0,1]\to [0,1]$ be a continuous monotonic function with $g(0)=0, g(1)=1$, which is used as the bijective connection function $y=g(x)$. The label $z$ is given by $z=\mathbf{1}_{[x-y>0]}$. In the domain of $(\mathcal{X},\mathcal{Y})$, the data $(x,y,z)$ is apparently separated by the line $x-y=0$. However, for either $\mathcal{X}$ or $\mathcal{Y}$, the set of points with label $z=1$ can be any union of countably many open intervals in $(0,1)$.

An illustrating example of such advantage is the following. Let $\mathcal{X}=\mathbb{R}$ and $\mathcal{Y}=\mathbb{R}^k$, we consider a distribution on $\mathcal{S}$, such that for any possible data point $(x,y,z)\in \mathcal{S}$, we have that $y=xv+y_0$ for some fixed $v,y_0\in \mathbb{R}^k$. The hypothesis classes we consider are, all $k$-degree polynomials for $\mathcal{G}$
$$
\mathcal{G}=\left\{g(x)=\sum_{i=0}^k x^i v_i|v_i\in \mathbb{R}^k\right\},
$$
and all hyperplanes for $\mathcal{F}$
$$
\mathcal{F}=\left\{f(x)=\textbf{sign}(x^{\top}v-c)|v\in \mathbb{R}^{k+1}, c\in \mathbb{R}\right\}.
$$
Take any sample $S$ with size $n\le k$. The worst case Gaussian average $\max_{g\in \mathcal{G}} G(\mathcal{F}(S(g)))$ can be as large as $\Omega(n)$, because the hypothesis class $\mathcal{F}$ is known to be able to shatter any $k$ points in $\mathbb{R}^{k+1}$ that are linearly independent, while the class $\mathcal{G}$ is expressive enough to contribute a worst-case $g$ that does map $X$ to a set of linearly independent points. However, it's possible that the learnt $\hat{g}$ is a low-dimensional polynomial. In particular, when it indeed learns the correct connection $g(x)=xv+y_0$, then the $n$ points $(x_1,\hat{g}(x_1)),...,(x_n,\hat{g}(x_n))$ are on the same line, and $G(\mathcal{F}(\hat{X},\hat{Y}))$ is just $O(\sqrt{n})$.

We note that the example doesn't contradict the results of \cite{maurer2006rademacher} \cite{tripuraneni2020theory}. It's known that in general $G(\mathcal{F}(X))=\tilde{O}(\sqrt{n d})$ where $d$ is the VC-dimension of $\mathcal{F}$. In this example, $d\ge k\ge n$, thus the worst-case value $\max_{g\in \mathcal{G}} G(\mathcal{F}(S(g)))$ actually matches the upper bound $\tilde{O}(\sqrt{n d})$. However, the term $G(\mathcal{F}(\hat{X},\hat{Y}))$ in our bound can be smaller by a factor of $\sqrt{n}$, proving that our instance-dependent bound is better. Informally, multimodal learning can be sensed as representation learning trained with explicit representations. 

$\mathcal{R}(\mathcal{G},S)=0$ with $g(x)=\theta^* x \in \mathcal{G}$ being the witness. To bound $\mathbb{E}[G(\mathcal{G}(X))]$, we notice that for any $k\le n$ number of distinct values $x_1,...,x_k\in (0,1]$,
$$
G(\mathcal{G}(\{x_1,...,x_k\}))\le \mathbb{E}_{\sigma}\left[ |\sum_{i=1}^k \sigma_i x_i| \right]=O(\sqrt{k})=O(\sqrt{n}).
$$
As a result, for any $X$ we have that $G(\mathcal{G}(X))=O(\sqrt{n})$, clearly $\mathbb{E}[G(\mathcal{G}(X))]=O(\sqrt{n})$ as well.

==> poster/defs.tex <==
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{definition}{Definition}[section]
%\newtheorem{example}[theorem]{Example}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{application}[theorem]{Application}
%\newtheorem{optimizationproblem}[theorem]{Optimization~Problem}

\newcommand{\todo}[1]{\textbf{\textcolor{red}{TODO: #1}}}

\DeclareMathOperator{\clip}{clip}
\def\norm#1{\mathopen\| #1 \mathclose\|}% use instead of $\|x\|$

\newcommand{\ellipsoid}{{\mathcal E}}
\newcommand{\sround}{\mathop{\mbox{\rm SmartRound}}}
\newcommand{\round}{\mathop{\mbox{\rm round}}}
\newcommand{\myspan}{\mathop{\mbox{\rm span}}}
\newcommand{\edges}{\mathop{\mbox{\rm edges}}}
\newcommand{\conv}{\mathop{\mbox{\rm conv}}}
\newcommand{\poly}{\mathop{\mbox{\rm poly}}}
\newcommand{\rank}{\mathop{\mbox{\rm rank}}}

\newcommand{\ignore}[1]{}
\newcommand{\equaldef}{\stackrel{\text{\tiny def}}{=}}
\newcommand{\equaltri}{\triangleq}
\newcommand{\tr}{\ensuremath{{\scriptscriptstyle\mathsf{T}}}}
\def\trace{{\bf Tr}}
\def\dist{{\bf P}}
\def\mydist{{\bf Q}}
\def\reals{{\mathbb R}}
%\newcommand\E{\mbox{\bf E}}
\newcommand\ball{\mathbb{B}}
\newcommand\var{\mbox{VAR}}
\newcommand\Lcal{\mathcal{L}}
\def\bzero{\mathbf{0}}

\def\Exp{\mathop{\mbox{E}}}
\def\mP{{\mathcal P}}
\def\risk{{\mbox{Risk}}}
\def\ent{{\mbox{ent}}}
\def\mG{{\mathcal G}}
\def\mA{{\mathcal A}}
\def\lhat{\hat{\ell}}
\def\Lhat{\hat{L}}
\def\ltil{\tilde{\ell}}
\def\Ltil{\tilde{L}}

\def\Ahat{\hat{\mathbf{A}}}

\def\bold0{\mathbf{0}}
\def\boldone{\mathbf{1}}
\def\boldp{\mathbf{p}}
\def\boldq{\mathbf{q}}
\def\boldr{\mathbf{r}}
\def\boldA{\mathbf{A}}
\def\boldI{\mathbf{I}}
\newcommand\mycases[4] {{
\left\{
\begin{array}{ll}
    {#1} & {#2} \\\\
    {#3} & {#4}
\end{array}
\right. }}
\newcommand\mythreecases[6] {{
\left\{
\begin{array}{ll}
    {#1} & {#2} \\\\
    {#3} & {#4} \\\\
    {#5} & {#6}
\end{array}
\right. }}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\be{\mathbf{e}}
\def\etil{\tilde{\mathbf{e}}}
\def\bk{\mathbf{k}}
\def\bu{\mathbf{u}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}

\def\bw{\mathbf{w}}
\def\ba{\mathbf{a}}
\def\bA{\mathbf{A}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bV{\mathbf{V}}
\def\bone{\mathbf{1}}


\def\xhat{\hat{\mathbf{x}}}
\def\xbar{\bar{\mathbf{x}}}
\def\vol{\mbox{vol}}
\def\trace{{\bf Tr}}
\def\Exp{\mathop{\mbox{E}}}
\newcommand{\val}{\mathop{\mbox{\rm val}}}
\renewcommand{\deg}{\mathop{\mbox{\rm deg}}}
%\newcommand{\eps}{\varepsilon}

% Macros for this chapter
\def\bone{\mathbf{1}}
\newcommand{\sphere}{\ensuremath{\mathbb {S}}}
\newcommand{\simplex}{\ensuremath{\Delta}}
\newcommand{\Ktil}{\ensuremath{\mathcal{\tilde{K}}}}
\def\mA{{\mathcal A}}
\newcommand{\rv}[1][t]{\ensuremath{\mathbf r_{#1}}}
\newcommand{\z}{\ensuremath{\mathbf z}}
\newcommand{\xtil}[1][t]{\ensuremath{\mathbf {\tilde{x}}_{#1}}}
\newcommand{\xv}[1][t]{\ensuremath{\mathbf x_{#1}}}
\newcommand{\xvh}[1][t]{\ensuremath{\mathbf {\hat x}}_{#1}}
\newcommand{\ftildeh}[1][t]{\ensuremath{\mathbf {\hat f}}_{#1}}
\newcommand{\xvbar}[1][t]{\ensuremath{\bar{\mathbf x}_{#1}}}
\newcommand{\xstar}{\ensuremath{\mathbf x^{*}}}
\newcommand{\xstarr}{\ensuremath{\mathbf x^{\star}}}
\newcommand{\yv}[1][t]{\ensuremath{\mathbf y_{#1}}}
\newcommand{\zv}[1][t]{\ensuremath{\mathbf z_{#1}}}
\newcommand{\fv}[1][t]{\ensuremath{\mathbf f_{#1}}}
\newcommand{\gv}[1][t]{\ensuremath{\mathbf g_{#1}}}
\newcommand{\qv}[1][t]{\ensuremath{\mathbf q_{#1}}}
\newcommand{\pv}[1][t]{\ensuremath{\mathbf p_{#1}}}
\newcommand{\ftilde}[1][t]{\ensuremath{\mathbf {\tilde f}_{#1}}}
\newcommand{\gtilde}[1][t]{\ensuremath{\mathbf {\tilde g}_{#1}}}
\newcommand{\lowtrace}{\mathcal{T}}

\newcommand{\ev}[1][i]{\ensuremath{\mathbf e_{#1}}}
\newcommand{\uv}{\ensuremath{\mathbf u}}
\newcommand{\ww}{\ensuremath{\mathbf w}}
\newcommand{\vv}{\ensuremath{\mathbf v}}
\newcommand{\A}[1][t]{\ensuremath{\mathbf A_{#1}}}
\newcommand{\Ftilde}[1][t]{\ensuremath{\mathbf {\tilde F}_{#1}}}
\newcommand{\Gtilde}[1][t]{\ensuremath{\mathbf {\tilde G}_{#1}}}
\newcommand{\hessum}[1][t]{\ensuremath{\boldsymbol{H}_{1:#1}}}
\newcommand{\reg}[1][t]{\ensuremath{\lambda_{#1}}}
\newcommand{\regsum}[1][t]{\ensuremath{\boldsymbol{\lambda}_{1:#1}}}
\newcommand{\bM}{\ensuremath{\mathcal M}}
%\newcommand{\F}{\ensuremath{\mathcal F}}
\newcommand{\ntil}{\tilde{\nabla}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\rhotil}{\tilde{\rho}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\mutil}{\tilde{\mu}}
\newcommand{\Atil}{\tilde{A}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\vtil}{\tilde{v}}
\newcommand\super[1] {{^{(#1)}}}
\newcommand\pr{\mbox{\bf Pr}}
\newcommand\av{\mbox{\bf E}}
\def\bb{\mathbf{b}}
%\def\bB{\mathbf{B}}
\def\bB{{B}}
%\def\bC{\mathbf{C}}
\def\bC{{C}}
\def\bS{{S}}
\def\be{\mathbf{e}}
\def\bu{\mathbf{u}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}
\def\bp{\mathbf{p}}
\def\bdelta{\mathbf{\delta}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bv{\mathbf{v}}
\def\ba{\mathbf{a}}
%\def\bA{\mathbf{A}}
\def\bA{{A}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bP{\mathbf{P}}
\def\bV{\mathbf{V}}
\def\sgn{\text{sgn}}
\def\eps{\varepsilon}
\def\epsilon{\varepsilon}
\def\tsum{{\textstyle \sum}}
\def\universal{{\sc Universal}\xspace}
\def\ogd{{\sc Online Gradient Descent}\xspace}


% modifiers
\newcommand{\obar}[1]{\overline{#1}}
\newcommand{\ubar}[1]{\underline{#1}}
\newcommand{\defeq}{\stackrel{\text{def}}{=}}

% brackets
\newcommand{\braces}[1]{\left\{#1\right\}}
\newcommand{\pa}[1]{\left(#1\right)}
\newcommand{\ang}[1]{\left<#1\right>}
\newcommand{\bra}[1]{\left[#1\right]}
\newcommand{\abs}[1]{\left|#1\right|}

% matrices, fractions, derivatives
\newcommand{\mat}[1]{\begin{matrix}#1\end{matrix}}
\newcommand{\pmat}[1]{\pa{\mat{#1}}}
\newcommand{\bmat}[1]{\bra{\mat{#1}}}
\newcommand{\sismat}[1]{\left\{\mat{#1}\right.}
\newcommand{\sm}[1]{\begin{smallmatrix}#1\end{smallmatrix}}
\newcommand{\psm}[1]{\pa{\sm{#1}}}
\newcommand{\bsm}[1]{\bra{\sm{#1}}}
\newcommand{\tci}[2]{\set{\,#1 \mid{} #2\,}}
\newcommand{\tcia}[2]{\ang{\,#1 \mid{} #2\,}}
\newcommand{\pfrac}[2]{\pa{\frac{#1}{#2}}}
\newcommand{\bfrac}[2]{\bra{\frac{#1}{#2}}}
\newcommand{\psfrac}[2]{\pa{\sfrac{#1}{#2}}}
\newcommand{\bsfrac}[2]{\bra{\sfrac{#1}{#2}}}
\newcommand{\der}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pder}[2]{\pfrac{\partial #1}{\partial #2}}
\newcommand{\sder}[2]{\sfrac{\partial #1}{\partial #2}}
\newcommand{\psder}[2]{\psfrac{\partial #1}{\partial #2}}
\newcommand{\case}[1]{\begin{cases}#1\end{cases}}

% operators
\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\Var}{\operatorname{Var}}
\DeclareMathOperator{\Cov}{\operatorname{Cov}}

% letters
\newcommand{\CC}{\mathbb{C}}
%\newcommand{\eps}{\varepsilon}


% theorems
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}

% environment shorthands
\newcommand{\eqn}[1]{\begin{equation}#1\end{equation}}


\DeclareMathOperator*\E{\mathbb{E}}
\newcommand\R{\mathbb{R}}
\newcommand\Sph{\mathbb{S}}
\newcommand\C{\mathbb{C}}
\newcommand\w{\mathbf{w}}
\newcommand\bias{\mathbf{b}}
\newcommand\ome{\mathbf{\omega}}
\newcommand\Y{\mathbf{Y}}
\newcommand\K{\mathbf{K}}
\newcommand\N{\mathcal{N}}
\newcommand\D{\mathcal{D}}
\newcommand\U{\mathcal{U}}
\newcommand\V{\mathcal{V}}
\newcommand\X{\mathcal{X}}
\newcommand\sig{\mathcal{\sigma}}
\newcommand\x{\mathbf{x}}
\newcommand\y{\mathbf{y}}
\newcommand\al{\boldsymbol{\alpha}}

\def\Pbb{\mathbb{P}}

\renewcommand\t{{\scriptscriptstyle\top}}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Astar}{\tilde{A}}
\DeclareMathOperator{\Bstar}{\tilde{B}}
\DeclareMathOperator{\Cstar}{\tilde{C}}
\DeclareMathOperator{\wstar}{\tilde{w}}
\DeclareMathOperator{\astar}{\tilde{a}}
\DeclareMathOperator{\bstar}{\tilde{b}}
\DeclareMathOperator{\cstar}{\tilde{c}}
\newcommand\wh{\widehat}
\newcommand\wt{\widetilde}
%\newcommand\eps{\varepsilon}
%\newcommand\veps{\varepsilon}
\newcommand\h{\hat}

\DeclareMathOperator{\MMD}{\mathrm{MMD}}

\newcommand\tl{\tilde}
%\newcommand\bar{\overline}
\newcommand\inner[1]{\langle #1 \rangle}
\newcommand\sign{\operatorname{sign}}
\newcommand{\Ds}{\mathcal{D}_{synth}}
\newcommand{\Dr}{\mathcal{D}_{real}}
\newcommand\indicator[1]{\ensuremath{\mathbf{1}_{#1}}}
\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand*\Diff[1]{\mathop{}\!\mathrm{d^#1}}


